An Empirical Analysis of Fairness Notions under Differential Privacy

Recent works have shown that selecting an optimal model architecture suited to the differential privacy setting is necessary to achieve the best possible utility for a given privacy budget using differentially private stochastic gradient descent (DP-SGD)(Tramer and Boneh 2020; Cheng et al. 2022). In light of these findings, we empirically analyse how different fairness notions, belonging to distinct classes of statistical fairness criteria (independence, separation and sufficiency), are impacted when one selects a model architecture suitable for DP-SGD, optimized for utility. Using standard datasets from ML fairness literature, we show using a rigorous experimental protocol, that by selecting the optimal model architecture for DP-SGD, the differences across groups concerning the relevant fairness metrics (demographic parity, equalized odds and predictive parity) more often decrease or are negligibly impacted, compared to the non-private baseline, for which optimal model architecture has also been selected to maximize utility. These findings challenge the understanding that differential privacy will necessarily exacerbate unfairness in deep learning models trained on biased datasets.

==> PPAI23New/abstract.tex <==
Recent works have shown that selecting an optimal model architecture suited to the differential privacy setting is necessary to achieve the best possible utility for a given privacy budget when using DP-SGD. In light of these findings, we empirically analyze how different fairness notions belonging to distinct classes of statistical fairness criteria (independence, separation and sufficiency) are impacted when one selects a model architecture that is suitable for DP-SGD and optimized for utility. Using standard datasets from ML fairness literature and a rigorous experimental protocol, we show that under these conditions, the differences across groups in the relevant fairness metrics (demographic parity, equalized odds and predictive parity) typically decrease or remain negligible compared to a non-private baseline, where the optimal model architecture was also selected to maximize utility. Our findings challenge the understanding that differential privacy will necessarily exacerbate unfairness in deep learning models trained on biased datasets.

==> PPAI23New/background.tex <==
% % This section provides an overview of the main concepts necessary to understand the present paper.

% % \subsection{Differential Privacy}
% % Differential Privacy is the flagship definition of data privacy. Differential Privacy ensures that approximately nothing can be learned about an individual whether she/he participates or not in a database. 
% % Differential Privacy defines a constraint on the processing of data such that the output of two adjacent databases is approximately the same. More formally: 

% % \begin{definition}
% % A randomized algorithm $M$ gives $(\epsilon, \delta)$-differential privacy, if for all databases $D$ and $D'$ differing on at most one element, and all $ S  \subseteq Range(M)$, $Pr[ M(D) \in S] \leq e^\epsilon Pr[ M(D') \in S] + \delta $ \citep{DBLP:journals/fttcs/DworkR14}.
% % \end{definition}

% % This condition encapsulates the crucial notion of indistinguishability of the results of a database manipulation whether someone participates or not in that database. The confidence parameter, $\epsilon$, is referred to as the privacy budget. Note that as $\epsilon$ decreases, the output of the mechanism becomes more private. The values of interest for $\delta$ are less than the inverse of any polynomial in the size of the database.
% % Any function, $M$, that satisfies the Differential Privacy condition can be used to generate data that guarantees the privacy of the individuals in the database. One interesting property of Differential Privacy is composability. If $M$ and $M'$ are $\epsilon$ and $\epsilon'$ differentially private, respectively, then their composition, $M \circ M'$, is ($\epsilon$ + $\epsilon$')-differentially private~\citep{DBLP:conf/tamc/Dwork08}. This property allows a user to create and combine many different mechanisms to achieve differential privacy.

% % \paragraph{R{\'e}nyi Differential Privacy}

% % R{\'e}nyi Differential Privacy (RDP)\citep{DBLP:conf/csfw/Mironov17} is a generalization of pure differential privacy that uses the R{\'e}nyi divergence of order $\lambda$ between two distributions $\mathcal{D}_{M(D)}$ and $D_{M(D')}$, where $M(.)$ is a mechanism applied to datasets $D$ and $D'$ that differ by one element. In RDP, the privacy parameter $\epsilon$ becomes a function $\epsilon(\lambda)$, rather than simply a scalar value. This variation offers a simple and precise composition property, allowing better control over the total privacy budget spent during multiple queries or operations.

% % \subsubsection{DP-SGD}
% % \citet{DBLP:conf/ccs/AbadiCGMMT016} developed an algorithm to insert differential privacy into the training procedure of a deep learning model. This method requires truncating the computed gradients and adding random noise to obfuscate the influence of a single input data on the final model. The training process can be defined as follows: first, a set of inputs, called lots, is processed by the model and the loss is computed; next, an array, composed of the gradients for each weight, is calculated with respect to the loss; then, the  gradients are clipped, returning the minimum value between the norm of the gradients and an upper bound defined as a hyperparameter of the differential privacy mechanism; finally, Noise, coming from a normal distribution, is added to the sum of clipped gradients with a variance proportional to the aforementioned upper bound and a noise multiplier parameter. The result is a sanitized version of the gradients, in which the influence of the input data is bounded, guaranteeing privacy. Consequently, the resulting model will have less accuracy than a comparable baseline model, trained without noise addition.

\section{Background}\label{sec:background}
\subsection{Differential Privacy}
Differential privacy (DP) is a rigorous mathematical framework for quantifying and limiting the amount of information that can be inferred about any input data point from the output of an algorithm~\cite{dwork2006calibrating,dwork2006our,dwork2014algorithmic}. Its strong privacy guarantees come from ensuring that the presence or absence of any single data point has a limited effect on the distribution of the algorithm's output. More formally, an algorithm $\mathcal{M}$ satisfies $(\varepsilon,\delta)$-differential privacy if for all set of outputs $S \subseteq \text{Range}(\mathcal{M})$ and for all datasets $D$ and $D'$ that differ on a single example:
\begin{equation*}
\Pr[\mathcal{M}(D) \in S] \leq e^\varepsilon \Pr[\mathcal{M}(D') \in S] + \delta,    
\end{equation*}
where $\varepsilon$ represents the privacy budget (smaller values indicating stronger privacy guarantees) and $\delta$ is the small probability of failure (typically $\delta \ll 1 / N$, where $N$ is the size of $D$~\cite{abadi2016deep}). At a high level, the $(\varepsilon, \delta)$-DP guarantees imply that the probability distribution of the model's outputs changes by at most a factor of $e^\varepsilon$ (with a small additional $\delta$ probability of failure) when trained on two separate datasets that differ by a single example. DP has several particularly useful properties. First, the composition of multiple algorithms with DP guarantees is still differentially private, i.e., if $\mathcal{M}$ and $\mathcal{M}'$ are $(\varepsilon,\delta)$-DP and $(\varepsilon',\delta')$-DP, respectively, then according to the basic composition theorem, $\mathcal{M} \circ \mathcal{M}'$ has in the worst case ($\varepsilon$~+~$\varepsilon'$, $\delta$~+~$\delta'$)-DP guarantees~\cite{dwork2006our, dwork2006calibrating}. Second, the output of any differentially private algorithm can be arbitrarily post-processed without any impact on its privacy guarantees. While other variants of DP exist that use slightly modified formulations (e.g., R{\'e}nyi Differential Privacy~\cite{mironov2017renyi}), $(\varepsilon,\delta)$-DP is presented for its simplicity.

\paragraph{DP-SGD.} As differential privacy was originally developed to be a general framework for privacy-preserving data analysis, it has been able to extend beyond its initial applications in private database queries to ML settings through various approaches, the most common of which is Differentially Private Stochastic Gradient Descent (DP-SGD)~\cite{abadi2016deep}. This technique adapts the standard SGD algorithm to provide DP guarantees for the trained model. The key modifications include:
\begin{enumerate}
    \item Per-example gradient clipping to bound the gradient calculation's sensitivity.
    \item Adding calibrated Gaussian noise to the aggregated gradients.
\end{enumerate}
By applying these operations and choosing $\sigma = \sqrt{2\log\frac{1.25}{\delta}} / \epsilon$, according to standard arguments~\cite{dwork2014algorithmic}, each step of DP-SGD is $(\epsilon,\delta)$-DP with respect to the batch. Moreover, for a training data of size $N$, batch size of size $B$, sampling ratio equal to $\alpha = B / N$, and an overall number of training steps $K = T J$, using the moments account~\cite{abadi2016deep} the algorithm has $(O(\epsilon\alpha\sqrt{K}),\delta)$-DP guarantees with respect to the training data for an appropriate choice of noise scale and gradient norm bound. In essence, this procedure guarantees the privacy of the training data (up to the $(\varepsilon,\delta)$-DP privacy budget) by limiting each individual data point's contribution to the model's learned parameters.

% \paragraph{R{\'e}nyi Differential Privacy.}
% R{\'e}nyi Differential Privacy (RDP)\cite{mironov2017renyi} is a generalization of pure DP that uses the R{\'e}nyi divergence of order $\lambda$ between two distributions $\mathcal{D}_{\mathcal{M}(D)}$ and $\mathcal{D}_{M(D')}$, where $M(.)$ is an algorithm applied to datasets $D$ and $D'$ that differ on a single example. In RDP, the privacy parameter $\epsilon$ becomes a function $\epsilon(\lambda)$, rather than simply a scalar value. This variation offers a simple and precise composition property, allowing better control over the total privacy budget spent during multiple queries or operations.


% % \subsubsection{DP-SGD}
% % \citet{DBLP:conf/ccs/AbadiCGMMT016} developed an algorithm to insert differential privacy into the training procedure of a deep learning model. This method requires truncating the computed gradients and adding random noise to obfuscate the influence of a single input data on the final model. The training process can be defined as follows: first, a set of inputs, called lots, is processed by the model and the loss is computed; next, an array, composed of the gradients for each weight, is calculated with respect to the loss; then, the  gradients are clipped, returning the minimum value between the norm of the gradients and an upper bound defined as a hyperparameter of the differential privacy mechanism; finally, Noise, coming from a normal distribution, is added to the sum of clipped gradients with a variance proportional to the aforementioned upper bound and a noise multiplier parameter. The result is a sanitized version of the gradients, in which the influence of the input data is bounded, guaranteeing privacy. Consequently, the resulting model will have less accuracy than a comparable baseline model, trained without noise addition.

\subsection{Fairness Notions}\label{secNotions}
In this section, we define the group fairness notions to be analyzed, which are drawn from three distinct classes of statistical non-discrimination criteria: independence, separation, and sufficiency~\cite{barocas-hardt-narayanan}. These notions pertain to the joint distributions of sensitive attributes, target labels, and predicted labels, and are expressed as conditional independence statements between these variables~\cite{castelnovo2022clarification}. We use demographic parity to represent independence, equalized odds to represent separation, and predictive parity to represent sufficiency, each of which is described in detail below. Given the subjective nature of fairness criteria selection for different use cases, we do not assess their specific relevance to the datasets in our analysis (see~\cite{makhlouf2021applicability} for a discussion on this topic). Instead, we focus on examining the effects of using DP-SGD to train ML models with respect to each criterion.

\paragraph{Demographic Parity.}
A classifier satisfies the demographic parity constraint when each subgroup receives a positive outcome at equal rates. More formally, this can be expressed as:
\begin{align}
P(\hat{Y} = 1 | A = a) = P(\hat{Y} = 1 | A = b ), \nonumber \: \forall a, b \in A \nonumber
\end{align}
where $\hat{Y}$ is the predicted label, and $A$ is the protected attribute indicating subgroup membership~\cite{barocas-hardt-narayanan}. Demographic parity aims to prevent the reinforcement of historical biases and can support underprivileged groups in the short term by enforcing a positive feedback loop. However, while demographic parity focuses on equal outcomes, it overlooks equality of treatment. This can lead to the issue of ``laziness''~\cite{makhlouf2021applicability,carey2022causal}, also known as ``self-fulfilling prophecy''~\cite{dwork2012fairness}, where a model correctly predicts true positives for privileged groups but randomly selects individuals from underprivileged groups until the proportion selected for each subgroup is equal. Additionally, demographic parity can be misapplied in contexts where disparities are legitimate and unrelated to protected attributes~\cite{dwork2012fairness}.

\paragraph{Equalized Odds.}
A classifier satisfies the equalized odds constraint when it has the same false positive rate and false negative rate for all subgroups. More formally, this can be expressed as:
\begin{align}
P(\hat{Y} = 1 | A = a, Y = y) = P(\hat{Y} = 1 | A = b, Y = y) \nonumber \\ 
\forall a, b \in A, y \in \{0,1\} \nonumber
\end{align}
where  $\hat{Y}$ is the predicted label, $A$ is the protected attribute, and $Y$ is the ground truth label~\cite{hardt2016equality}. Unlike demographic parity, equalized odds uses the ground truth label to ensure equality of treatment, thereby eliminating the laziness issue mentioned above. However, equalized odds can be problematic when the target variable is inherently biased (e.g., a university admissions process that has historically discriminated against a particular group), as this can result in the propagation of existing biases~\cite{castelnovo2022clarification}.

\paragraph{Predictive Parity.}
A classifier satisfies the predictive parity constraint when it has the same precision for all subgroups. More formally, this can be expressed as:
\begin{align}
P(Y = 1 | A = a, \hat{Y} = 1) = P( Y = 1 | A = b, \hat{Y} = 1 ) \nonumber \\ 
\forall a, b \in A \nonumber
\end{align}
where  $Y$ is the ground truth label, $A$ is the protected attribute, and $\hat{Y}$ is the predicted label~\cite{chouldechova2017fair}. Contrary to demographic parity and equalized odds, predictive parity evaluates subgroups based on the model's predictions ($\hat{Y}$) rather than the actual outcomes ($Y$). This approach is often more practical, as prediction-based metrics can be assessed immediately after the model makes decisions, while true outcomes can only be observed in retrospect~\cite{castelnovo2022clarification}

As a general point, it is important to recognize that independence, separation, and sufficiency cannot all hold simultaneously \cite[Chapter 3]{barocas-hardt-narayanan}. This means that in datasets like those used in this paper, where the sensitive attributes are correlated with the target label, attempting to enforce more than one fairness criterion may lead to no feasible solution or a trivial model that performs poorly.

\subsection{Related Work}
In this section, we review existing work that addresses fairness concerns in the context of differential privacy.

\citet{bagdasaryan2019differential} investigates the impact of DP-SGD on underrepresented groups using several image and text datasets. The study finds the data from underrepresented subgroups produces larger gradients, causing the clipping operation to disproportionately limit their influence on the learned model. It is also shown that the random noise introduced by DP-SGD has a more significant impact on these groups. However, in some experiments, group membership is confused with class labels, and underrepresented groups are artificially created through under-sampling. The authors do not address how differential privacy impacts specific fairness notions.

\citet{pujol2020fair} examines fair allotment and decision rule problems using differential privacy. The study shows that the noise introduced by strong privacy guarantees leads to disparate decision errors for minority groups. Notably, the empirical analysis employs extremely small privacy budgets (on the order of $10^{-5}$). 

\citet{xu2021removing} proposes a DP-SGD approach that assigns an adaptive gradient clipping norm per group, aiming to achieve uniform accuracy loss across groups (or classes). The experiments do not explore the impact of this approach on other fairness notions.

\citet{tran2021fairness} evaluates excessive risk as a fairness notion in the context of privacy protection using the ensemble method PATE~\cite{papernot2018scalable}. The study analyzes how various model parameters influence the excessive risk difference across groups and demonstrates potential mitigation strategies for disparate effects by employing soft labels.

\citet{jagielski2019differentially} propose optimization procedures for achieving equalized odds under differential privacy. The work establishes theoretical bounds on the trade-offs between accuracy, privacy, and equalized odds, howing that stricter privacy constraints can increase fairness violations. Experimental results are presented to support this claim.

\citet{ganev2022robin} demonstrate the disparate impact of differential privacy on generative models with respect to minority and majority groups. This impact either reduces or increases the gap between demographic groups in the generated synthetic data, affecting both their proportions relative to the real data and the accuracy of downstream classification tasks.

\citet{cheng2022dpnas} showed that model utility (measured by test accuracy) is significantly improved when a targeted search for the best network architecture is conducted during training with DP-SGD. However, it is important to note that the privacy budget values reported in \cite{cheng2022dpnas} do not appear to account for potential privacy leakage during the architecture search process itself, as discussed in \cite{papernot2022hyperparameter}.

==> PPAI23New/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
Previous research has suggested that training deep learning models with differential privacy has a disparate impact on accuracy for underprivileged groups. While this observation may hold true when using DP-SGD with an existing non-private model configuration, our experiments show that this is not always the case. Specifically, identifying a model architecture and training hyperparameters suited to the DP setting appears to mitigate many of the previously observed issues with utility metrics and, in fact, often improves fairness when evaluated using standard fairness measures such as demographic parity, equalized odds, and predictive parity. However, our conclusions are based solely on tabular datasets commonly used in ML fairness research. Future work should explore whether these findings hold for datasets outside the tabular domain, such as those used to train language and vision models. Additionally, a deeper understanding of the mathematical relationship between DP-SGD and these fairness notions could provide greater insight into the effects at play. Overall, this research highlights the potential to balance utility with various Responsible AI principles, demonstrating that both can be effectively addressed in certain contexts.

==> PPAI23New/experiments.tex <==
\section{Experiments}\label{sec:experiments}
\begin{table*}[ht!]
\centering
\small
\begin{tabular}{c c ccc}
    \toprule
    Dataset & Metric  &  Baseline & Baseline + DP & Best DP Model \\
    \midrule
\multirow{4}{*}{Adult}
      & Overall AUC	 &	 \textbf{0.9056} $\pm$ 0.0011 &	 0.8476 $\pm$ 0.0073 &	 0.9005 $\pm$ 0.0009 \\
	 & AUC Difference	 &	 \textbf{0.1264} $\pm$ 0.0249 &	 0.2226 $\pm$ 0.0556 &	 0.1841 $\pm$ 0.0599 \\
	 & Demographic Parity Difference	 &	 0.2750 $\pm$ 0.0155 &	 0.4683 $\pm$ 0.0612 &	 \textbf{0.2375} $\pm$ 0.0207 \\
	 & Equalized Odds Difference	 &	 \textbf{0.7845} $\pm$ 0.0492 &	 0.8005 $\pm$ 0.0472 &	 0.8000 $\pm$ 0.0000 \\
	 & Predictive Parity Difference	 &	 0.9400 $\pm$ 0.0966 &	 \textbf{0.7567} $\pm$ 0.1933 &	0.8000 $\pm$ 0.000 \\
    \addlinespace
    \hline
    \addlinespace
\multirow{4}{*}{ACS Inc.}
      & Overall AUC	 &	 \textbf{0.8878} $\pm$ 0.0011 &	 0.8155 $\pm$ 0.0045 &	 0.8820 $\pm$ 0.0008 \\
	 & AUC Difference	 &	 0.2546 $\pm$ 0.0569 &	 0.3498 $\pm$ 0.0867 &	 \textbf{0.2225} $\pm$ 0.0219 \\
	 & Demographic Parity Difference	 &	 0.4223 $\pm$ 0.0613 &	 0.6105 $\pm$ 0.1234 &	 \textbf{0.2556} $\pm$ 0.0490 \\
	 & Equalized Odds Difference	 &	 0.4360 $\pm$ 0.0780 &	 0.8499 $\pm$ 0.1656 &	 \textbf{0.3756} $\pm$ 0.0019 \\
	 & Predictive Parity Difference	 &	 \textbf{0.3550} $\pm$ 0.0518 &	 0.7882 $\pm$ 0.2009 &	 0.4032 $\pm$ 0.0271 \\
    \addlinespace
    \hline
    \addlinespace
\multirow{4}{*}{ACS Emp.}  
 & Overall AUC	 &	 \textbf{0.8837} $\pm$ 0.0011 &	 0.8110 $\pm$ 0.0062 &	 0.8702 $\pm$ 0.0013\\
	 & AUC Difference	 &	 0.3401 $\pm$ 0.0875 &	 0.3134 $\pm$ 0.0653 &	 \textbf{0.2073} $\pm$ 0.0480\\
	 & Demographic Parity Difference	 &	 0.4383 $\pm$ 0.0805 &	 0.5317 $\pm$ 0.1561 &	 \textbf{0.3154} $\pm$ 0.0359\\
	 & Equalized Odds Difference	 &	 0.5884 $\pm$ 0.1360 &	 0.6623 $\pm$ 0.1701 &	 \textbf{0.2874} $\pm$ 0.0534\\
	 & Predictive Parity Difference	 &	 0.5534 $\pm$ 0.0998 &	 0.4833 $\pm$ 0.1296 &	 \textbf{0.2968} $\pm$ 0.0674\\
    \addlinespace
    \hline
    \addlinespace
\multirow{4}{*}{LSAC}
	 & Overall AUC	 &	 \textbf{0.8343} $\pm$ 0.0029 &	 0.7755 $\pm$ 0.0125 &	 0.7962 $\pm$ 0.0077 \\
	 & AUC Difference	 &	 0.0435 $\pm$ 0.0056 &	 \textbf{0.0422} $\pm$ 0.0142 &	 0.0575 $\pm$ 0.0128 \\
	 & Demographic Parity Difference	 &	 0.3064 $\pm$ 0.0653 &	 0.2007 $\pm$ 0.0437 &	 \textbf{0.1687} $\pm$ 0.0151 \\
	 & Equalized Odds Difference	 &	 0.2548 $\pm$ 0.0862 &	 0.2853 $\pm$ 0.0467 &	 \textbf{0.1975} $\pm$ 0.0722 \\
	 & Predictive Parity Difference	 &	 \textbf{0.1688} $\pm$ 0.0485 &	 0.2202 $\pm$ 0.0061 &	 0.2197 $\pm$ 0.0082 \\
    \addlinespace
    \hline
    \addlinespace
\multirow{4}{*}{Compas}
      & Overall AUC	 &	 \textbf{0.6895} $\pm$ 0.0041 &	 0.5349 $\pm$ 0.0359 &	 0.6863 $\pm$ 0.0030 \\
	 & AUC Difference	 &	 0.1162 $\pm$ 0.0273 &	 0.1295 $\pm$ 0.0390 &	 \textbf{0.0824} $\pm$ 0.0264 \\
	 & Demographic Parity Difference	 &	 0.5101 $\pm$ 0.0209 &	 \textbf{0.3322} $\pm$ 0.1331 &	 0.3694 $\pm$ 0.0230 \\
	 & Equalized Odds Difference	 &	 0.5592 $\pm$ 0.0476 &	 0.3905 $\pm$ 0.1356 &	 \textbf{0.3726} $\pm$ 0.0375 \\
	 & Predictive Parity Difference	 &	 0.3347 $\pm$ 0.0749 &	 \textbf{0.3009} $\pm$ 0.1052 &	 0.3168 $\pm$ 0.0467 \\
    \addlinespace  
    \bottomrule
\end{tabular}
\caption{Mean and standard deviation values are reported for 10 training runs of the best model configurations. The difference metrics represent the largest disparity for a given metric between any two subgroups in the dataset. The total privacy budget is $\varepsilon = 27$ for both the {\it Baseline + DP} and {\it Best DP} models.\label{tabMetrics}}
\end{table*}

Table~\ref{tabMetrics} shows our results on the five datasets for each of the relevant metrics: Overall AUC, Maximum AUC Difference, Maximum Demographic Parity Difference, Maximum Equalized Odds Difference, and Maximum Predictive Parity Difference. As explained in Section~\ref{dp-fairness:evaluation}, lower values for all ``difference'' metrics indicate better performance. The large values for all the differences in the \textit{Baseline} model column confirm the presence of biases in the datasets. While there is no universal scale for measuring sufficiency, separation, and independence, the differences across groups are significant enough to suggest that, in most cases, this level of disparity would be unacceptable, requiring fairness interventions to reduce disparities based on the chosen fairness criterion for each dataset. Our goal is to observe how these fairness metrics are impacted by the use of DP-SGD. Group-specific metrics for each dataset are provided in Appendix~\ref{app:group-specific}.

We observe that the {\it Best DP Model} outperforms the {\it Baseline + DP} model across nearly all metrics and datasets. Although we do not perform any additional fine-tuning (e.g., adjusting the learning rate) for the {\it Baseline + DP} models, it is still surprising how poorly they perform, especially considering that they use a much larger privacy budget of $\varepsilon = 27$ for training the final model, compared to $\varepsilon = 5$ for the {\it Best DP Model}. This difference in performance serves as further evidence that finding the best-performing model architecture and hyperparameters is essential in the DP setting. Moreover, the {\it Best DP Model} maintains strong Overall AUC scores compared to the \textit{Baseline} models, with decreases typically within 0.01, and a maximum decrease of 0.0381 on the LSAC dataset. 

In terms of fairness metrics, instead of exacerbating subgroup differences, the {\it Best DP Model} actually reduces bias more often than both the \textit{Baseline} and {\it Baseline + DP} models. The clearest examples of this are seen in the ACS Income and ACS Employment datasets, where the Overall AUC is nearly equal to the non-private baselines, and all group disparities have significantly decreased. In contrast, we do not observe substantial reductions in disparities for the Adult dataset, but training with DP-SGD does not appear to worsen biases. Overall, compared to the \textit{Baseline} model, the {\it Best DP Model} reduces disparities for the AUC Difference on three datasets, for the Demographic Parity Difference on all five datasets, for the Equalized Odds Difference on four datasets, and for the Predictive Parity Difference on three datasets.

While this analysis has been empirical, one can hypothesize that the noise and gradient clipping introduced by DP-SGD may act as a regularization effect, potentially enhancing the private model's generalization capabilities. This hypothesis is supported by group-specific metrics evaluated on the Cartesian product of the sensitive attributes for sex and race (see Appendix~\ref{app:intersection}), where the {\it Best DP Model} often assigns positive outcomes more frequently to underprivileged (or minority) groups. However, a more formal analysis along the lines of~\citet{tran2021differentially} is required before drawing any definitive conclusions.

==> PPAI23New/intro.tex <==
\section{Introduction}
Due to bias frequently present in the data used for machine learning (ML), systems responsible for high-stakes decisions---such as hiring, healthcare, social benefit allocation, and admissions to higher education---often produce unfair outcomes or perpetuate harmful biases against underprivileged groups~\cite{chouldechova2018frontiers,barocas-hardt-narayanan,mehrabi2021survey}. This concern has motivated substantial research efforts aimed at defining fairness notions, developing interventions in ML training to align with those notions, and applying these approaches across various datasets in supervised learning settings ~\cite{feldman2015certifying,hardt2016equality,zafar2017fairness_www,zafar2017fairness_aistats}. However, fairness is not the only consideration (beyond task-specific model utility) that ML models must take into account. They are also subject to membership inference attacks (MIAs), where an adversary attempts to infer whether specific input examples were used to train the model~\cite{shokri2017membership,hilprecht2019monte}. As differential privacy (DP) is one of the primary defenses against privacy attacks, researchers have begun examining its impact on fairness~\cite{bagdasaryan2019differential,xu2020removing,chang2021privacy,noe2022exploring}. These studies have generally shown that the accuracy reduction caused by DP tends to disproportionately affect underprivileged groups.
% % and other aspects of Responsible AI~\cite{song2019privacy,rice2020overfitting,shokri2021privacy,pawelczyk2023privacy}. Regarding fairness specifically, 
% Alternatively, we show that privacy protection does not always have a negative effect when it comes to disparities across groups. 

In parallel to examining DP’s impact on fairness, other research has focused on improving the utility-privacy trade-off inherent in differentially private stochastic gradient descent (DP-SGD). Recent work has demonstrated that model utility for a certain ($\varepsilon, \delta$)-DP privacy level can be increased significantly by selecting model architectures and training hyperparameters tailored to the unique aspects of DP-SGD, rather than simply applying DP-SGD to the best-performing non-private model~\cite{tramer2020differentially,cheng2022dpnas,de2022unlocking,kurakin2022toward}. Despite these findings, prior studies examining the impact of DP on fairness have generally taken the latter approach, applying DP-SGD to non-optimized models. As a result, these analyses have been conducted using private models that perform substantially worse than their non-private baselines, potentially leading to misleading conclusions. Several other concerns with existing analyses include: (1) the exclusive use of utility-based metrics to evaluate disparate impact, without considering established fairness notions; (2) the exclusion of tabular datasets derived from real-world situations, which are typically studied in ML fairness literature; (3) the removal of small minority groups and their intersections from fairness analysis, which is problematic because sensitive attributes, such as sex and race, have been collected at a level of granularity to include them, indicating their presence in real-world settings.

This paper presents the first exploration of DP-SGD's impact on fairness using ML model architectures and hyperparameters specifically optimized for the DP-SGD setting. To identify the private and non-private models with maximum possible utility, an exhaustive grid search is conducted over a broad range of model design and hyperparameter configurations. In addition to utility-based metrics, differences in demographic parity, equalized odds, and predictive parity across groups are measured using k-fold cross-validation on five commonly studied ML fairness datasets, while retaining naturally occurring minority groups in the data. Ultimately, we observe that selecting model and training configurations tailored to DP-SGD typically reduces or maintains negligible differences across groups in relevant fairness metrics, compared to the non-private baseline. These findings suggest that, contrary to previous reports, DP-SGD does not systematically amplify disparities across groups, particularly when fairness is evaluated using established fairness notions and highly-studied tabular ML fairness datasets.

The remainder of this paper is organized as follows. Section~\ref{sec:background} provides the necessary background on DP and fairness notions for understanding our contributions and discusses related work on the interplay between these two domains. Section~\ref{sec:methodology} details the ML fairness datasets, the model architecture and training hyperparameter configurations explored, and the privacy-preserving model selection process. Section~\ref{sec:experiments} presents the experimental results and provides commentary on the findings. Finally, Section~\ref{sec:conclusion} concludes the paper.

% % By using datasets typically examined in ML fairness research, we observed that by selecting the optimal model architecture with DP-SGD, either the fairness metrics are negligibly impacted or (more often) the differences across groups decrease, when compared to the non-private baseline, for which optimal model architecture and hyperparameter search has also been conducted for reaching maximum utility (represented by the ROC AUC score). 

% % Building on these results, we show empirically that differential privacy does not systematically amplify disparities across groups, when we examine certain fairness notions. We measured selected indicators supporting fairness notions that belong to opposing statistical non-discrimination criteria: independence, separation and sufficiency, using a rigorous experimental protocol.

% % Another important differentiation in this work is that we did not exclude minorities from the analysis, nor outliers, while it may be a widespread practice in data science and in (machine learning) research. We measure the fairness disparities in realistic situation where the fairness indicators on all minority groups and their intersections, as we consider two protected attributes for each dataset (race and sex). 

% % We draw our conclusions after performing exhaustive grid-search, for the private and non-private settings (including activation function, optimizer, number of hidden layers, dropout probability, learning rate, \ldots). 
% % The private grid search procedure uses randomization, consuming privacy budget.  
% % We measure key group fairness metrics using k-fold cross validation for each dataset to measure equalized odds, predictive parity and demographic parity differences.

% % We selected ROC AUC score because it is robust to class imbalance and also independent of a decision threshold. We observed that the ROC AUC score on the test set remains close for the best private and non-private models. 
% % The fact that we evaluate utility only, allows us to compare to previous research,  which simply incorporate a DP-SGD optimizer to the best non-private baseline architecture that have found that DP-SGD disparately impacts model's accuracy. 

==> PPAI23New/methodology.tex <==
\section{Methodology}\label{sec:methodology}

\subsection{Datasets}\label{secDatasets} 
To assess the real-world impact of DP-SGD on fairness, we used tabular datasets with demographic information that are widely used in ML fairness research~\cite{feldman2015certifying,zafar2017fairness_aistats,chouldechova2017fair,zafar2017fairness_www,barocas-hardt-narayanan,xu2020removing,lahoti2020fairness,chang2021privacy,ganev2022robin,wang2022towards,ezzeldin2023fairfed}. These datasets contain various types of biases in the relationships between sensitive features and the target variable.

\paragraph{Adult:} The UCI Adult dataset~\cite{Dua:2019} contains 49,531 income survey records from the 1994 U.S. census. For our classification task, we use the binarized ``income'' feature as the target variable, predicting whether an individual's income exceeds \$50k per year. The dataset also includes features such as sex, race, age, education, occupation, and marital status, among others.

\paragraph{ACS Income:} The ACS Income dataset~\cite{ding2021retiring} is a more recent alternative to the UCI Adult dataset, addressing certain limitations related to employment status and income reporting. It uses data from the years 2014-2018 and contains 1,599,229 data points. The dataset includes the same features as the Adult dataset, along with additional metadata such as geographical information. The task remains to predict whether an individual's income exceeds \$50k per year. For our analysis, we use a 10\% sample of the ACS survey results from California in 2018.

\paragraph{ACS Employment:} The ACS Employment dataset~\cite{ding2021retiring} is derived from the American Community Survey released by the U.S. Census Bureau, with the prediction target being whether an individual was employed during the year of data collection. We use 10\% of the survey results for California in 2018. The dataset includes features such as educational attainment, marital status, citizenship, and parental employment status, among others.

\paragraph{LSAC.} The Law School dataset~\cite{wightman1998lsac} is from the Law School Admissions Council’s National Longitudinal Bar Passage Study, aimed at predicting whether a candidate would pass the bar exam. It includes law school admission records with features such as gender, race, family income, and GPA-derived metrics. The classification target is the binary feature “isPassBar.”

\paragraph{COMPAS.} The COMPAS dataset~\cite{angwin2016machine} for recidivism risk prediction includes records of convicted individuals, along with their criminal history and demographic features such as gender and race. We use the binary outcome of whether the offender was re-arrested as the target variable for classification. Note that a positive outcome (True) represents an undesirable result. Additionally, the majority group (Black Males) has higher positive rates.

In each of these datasets, fairness and privacy are genuine concerns, as the prediction tasks can be applied in critical domains and the features include sensitive attributes. When specifically considering the privacy risks associated with MIAs, the inclusion of an individual in most of these datasets could potentially reveal private information. For example, in the COMPAS dataset, inclusion indicates that an individual has been convicted of a crime, and in the ACS Employment dataset, one could filter the data to only include non-citizens to predict their unemployment, where inclusion in this segment would reveal that the individual is not a citizen.

\subsection{Training}\label{dp-fairness:training}
During training, we retain all protected attributes (i.e., sex and race) in each dataset.\footnote{We initially conducted a second set of experiments where we removed the two sensitive attributes, sex and race, which are used to construct subgroups for evaluating fairness. However, by doing so, we observed a significant decline in the AUC score across all datasets and settings, making it difficult to accurately assess the impact of DP-SGD on fairness metrics.} This approach aligns with the seminal work by~\citet{dwork2012fairness}, which demonstrates that removing protected attributes does not mitigate bias, as these attributes are often correlated with proxy features---this is indeed the case for the five datasets we consider. We also transform all categorical features into one-hot encoded vectors and standardize all numerical features to have zero mean and unit variance for each dataset. 

To conduct our grid search, we first define a template for a feed-forward neural network, consisting of an input block, a variable number of hidden blocks, and a final softmax layer. Each input and hidden block contains a linear layer, normalization, and dropout, as shown in Figure~\ref{figModel} in Appendix~\ref{app:model-architecture}.

Using this model architecture, we perform a 5-fold cross-validation grid search on each dataset to find the best configurations, aiming to maximize overall model utility. The following list presents the configuration options considered in our search:
\begin{itemize}
    \item[$\bullet$] Learning rate: $10^{-5}, 10^{-4}, 10^{-3}, 10^{-2}$
    \item[$\bullet$] Dropout probability: $0.0, 0.1, 0.2$
    \item[$\bullet$] Number of hidden blocks: $1$ to $3$
    \item[$\bullet$] Batch size: $256, 512$
    \item[$\bullet$] Activation functions: Relu, Tanh
    \item[$\bullet$] Optimizers: Adam, SGD
    \item[$\bullet$] Maximum gradient clipping norm (only relevant for DP): $10^{-3}, 10^{-2}, 10^{-1}$
\end{itemize}
Following previous work~\cite{lahoti2020fairness}, we use the AUC score (area under the receiver operating characteristic (ROC) curve) to quantify utility, which is calculated using false positive rates and true positive rates at different decision thresholds (i.e., the value above which a prediction is considered positive in a binary classification). This metric is suitable for fairness-related tasks because it is insensitive to class imbalance. Moreover, optimizing for utility enables us to compare our results to prior works that apply DP-SGD to the best non-private configuration, and to assess the fairness of private models when achieving fairness is not an explicit goal. We perform the hyperparameter search separately for both DP and non-DP settings using the distributed training framework provided by \textit{Ray Tune}\footnote{\url{https://docs.ray.io/en/latest/tune/index.html}}, with DP-SGD applied via the \textit{Opacus}~\cite{opacus} library. All experiments are run using 2 GPUs on an NVIDIA DGX server. 
% To find the best-performing models in all settings, we perform the search for each of the datasets under four different setups: (1) with and without DP; (2) with and without the protected attributes (sex and race). 

The ($\varepsilon, \delta$)-DP budget for a single run of training with DP-SGD is set to $\varepsilon = 5$ and $\delta = 1 / N$, where $N$ is the size of the training data (a smaller $\varepsilon$ indicates stronger privacy protections). To achieve the desired $\varepsilon$ value, the privacy cost at each iteration is calculated~\cite{abadi2016deep}, with training continuing until the privacy budget is exhausted. Using the basic composition theorem of DP (see Section~\ref{sec:background}), the total privacy cost is estimated at $\varepsilon = 20$, as each of the five training splits is used four times for training (and once for validation). Additionally, the randomized hyperparameter search incurs an extra cost of $\varepsilon = 2$~\cite[Theorem 6]{papernot2022hyperparameter}, and training the final model after the search is complete adds another $\varepsilon = 5$. Thus, the total privacy budget for our procedure is conservatively estimated at $\varepsilon = 27$.

The last step in our procedure is to train models for each dataset in the following three settings: (1) Baseline, which corresponds to training with the best-performing non-private model configuration; (2) Baseline + DP, which uses the Baseline configuration and trains the model with DP-SGD---this mirrors most previous research, where DP-SGD is applied to the baseline model with little or no adjustment (e.g., minor changes to the learning rate); and (3) Best DP Model, which corresponds to training with DP-SGD and the best-performing private model configuration. As a final point, while the overall privacy budget for the {\it Best DP Model} is $\varepsilon = 27$, only $\varepsilon = 5$ is used for training the final model, as the remaining $\varepsilon = 22$ was consumed during the grid search. To ensure a fair comparison, the {\it Basline + DP} model, which does not involve a grid search, is trained using the full privacy budget of $\varepsilon = 27$.

% Here, we use a differential privacy budget (epsilon) equivalent to $27$ for each privacy-preserving version. That is, we explicitly set $\epsilon = 27$ for the {\it Basline + DP} models, whereas we set it to $\epsilon = 5.0$ for the {\it Best DP model} settings, and account for the privacy budget spent during the hyperparameter search phase. 

% Next, we trained models for each of the datasets using the best configuration for three settings: {\it Baseline}, without privacy protection; {\it Baseline+DP} which is the baseline model configuration with the addition of differential privacy;  and {\it Best DP Model} ). It is important to remark that the {\it Baseline+DP} case, we did not adjust any other hyperparameters, and used the privacy budget $\epsilon= 27$. Using the default model with differential privacy approximates what has occurred in most previous research, where differential privacy was added to the baseline models with minor adjustments, such as batch size or learning rate.

\subsection{Evaluation}\label{dp-fairness:evaluation}
We evaluate fairness based on the intersection of subgroups formed by all sex and race categories, which are the protected attributes present in each of the five datasets analyzed. This method enables a more accurate understanding of how underrepresented groups are impacted by private classifiers, in contrast to previous works that create artificial minority groups by undersampling certain classes (e.g., reducing the occurrence of class ``8'' in MNIST~\cite{bagdasaryan2019differential}), which has little relevance to real-world scenarios.

As outlined in Section~\ref{sec:background}, we consider three fairness metrics, each corresponding to a statistical fairness criterion: demographic parity (independence), equalized odds (separation), and predictive parity (sufficiency). These metrics are calculated using the \textit{Fairlearn} library~\cite{kulshrestha2021fairlearn}. Following previous work~\cite{lahoti2020fairness}, we focus on utility and fairness metrics for the worst-performing subgroup. Specifically, for the AUC and each fairness metric, we calculate the difference between the best-performing and worst-performing subgroups, which captures the largest disparity in the dataset. The closer these ``difference'' values are to $0$, the fairer the model is with respect to that metric. While the AUC is calculated across various decision thresholds, calculating the fairness metrics requires selecting a specific threshold to obtain a single set of predictions. In this case, we set the decision threshold to $0.5$ for all datasets. All metrics are evaluated on a hold-out test set (i.e., not used during the 5-fold cross-validation), with the results representing the mean values from 10 independent training runs.
